Provably Robust Blackbox Optimization for Reinforcement Learning

Interest in derivative-free optimization (DFO) and "evolutionary strategies" (ES) has recently surged in the Reinforcement Learning (RL) community, with growing evidence that they can match state of the art methods for policy optimization problems in Robotics. However, it is well known that DFO methods suffer from prohibitively high sampling complexity. They can also be very sensitive to noisy rewards and stochastic dynamics. In this paper, we propose a new class of algorithms, called Robust Blackbox Optimization (RBO). Remarkably, even if up to $23\%$ of all the measurements are arbitrarily corrupted, RBO can provably recover gradients to high accuracy. RBO relies on learning gradient flows using robust regression methods to enable off-policy updates. On several MuJoCo robot control tasks, when all other RL approaches collapse in the presence of adversarial noise, RBO is able to train policies effectively. We also show that RBO can be applied to legged locomotion tasks including path tracking for quadruped robots.

==> experiments.tex <==
\section{Experiments}
\label{sec:exp}


We conducted an exhaustive analysis of the proposed class of RBO algorithms on the following $\mathrm{OpenAI}$ $\mathrm{Gym}$ \cite{Gym} 
benchmark RL tasks: $\mathrm{Swimmer}$, $\mathrm{HalfCheetah}$, $\mathrm{Hopper}$, $\mathrm{Walker2d}$, $\mathrm{Humanoid}$ and $\mathrm{Pusher}$. 
We also used RBO to learn policies for the quadruped locomotion tasks (see: Section \ref{locomotion}) on real robots.
We tested both large noise settings, where as many as $25\%$ of all the measurements were corrupted and heavily
underconstrained settings, where the number $k$ of chosen perturbations per epoch satisfies $k \ll d$.
In these settings we still learned good quality policies with a small number of rollouts, whereas other methods either failed or needed more perturbations.
We trained locomotion policies for the quadruped robot in the PyBullet simulator (\cite{coumans}).
% The attached video contains a demonstration of the real quadruped minitaur robot walking and using stable policies trained by $\mathrm{RBO}$ as 
% well as videos from simulators for many of the tasks considered here.

Our main focus is to compare with other ES methods, in particular the state-of-the-art Augmented Random Search ($\mathrm{ARS}$) algorithm from \cite{horia}. 
ARS can be easily adjusted to different policy architectures, is characterized by lower sampling complexity than other ES algorithms and was showed to 
outperform other algorithms such as \cite{ES} on many different robotics tasks. This is possible due to the use of various efficient ES heuristics such as state 
and reward renormalization as well as perturbation filtering methods to substantially lower sampling complexity. ARS was also used to train quadruped locomotion tasks in \cite{atil}. 
Additionally, we added a comparison with non-ES policy gradient methods such as
$\mathrm{PPO}$ and $\mathrm{TRPO}$, even though this class uses MDP-structure of the RL blackbox function $F$ under consideration that RBO and $\mathrm{ARS}$ are agnostic to.

We tested two policy architectures: linear (on its own as for some $\mathrm{mujoco}$ tasks or as a part of larger hybrid policy
as for quadruped locomotion tasks) and nonlinear with two hidden layers, each of size $h=41$, with $\mathrm{tanh}$ nonlinearities and with connections encoded by low displacement rank ($\mathrm{LDR}$) Toeplitz matrices from \cite{stockholm}.
Below we will refer to them as: linear and $\mathrm{LDR}$/nonlinear policies respectively.

On some plots we presented different variants of the $\mathrm{RBO}$ algorithm, whereas in other we showed one (e.g. if all where giving similar training curves or a particular version
was most suitable as LP-decoding for the overconstrained setting with substantial noise). Presented results were obtained using dynamic trust region method with $\tau=5\%$.


\input{minitaur_walking}
\input{minitaur_path_tracking}
\input{mujoco}












==> gradient-recovery.tex <==
\section{Robust Blackbox Optimization Algorithm}
\label{sec:gradient-recovery}

$\mathrm{RBO}$ relies on the fact that by using different directions defining perturbed policies, one can obtain good estimates of the dot-product of the gradient $\nabla F(\theta)$
of the RL blackbox function $F$ in a given point $\theta$ with vectors defined by these directions, simply by performing rollouts of these perturbed policies and collecting obtained rewards. 
If $F$ is not differentiable, the notion of the gradient should be replaced by that of a smoothing of $F$ (applied on a regular basis to optimize non-convex non-differentiable functions, 
see \cite{nesterov}), but since the analysis will be completely similar, from now one without loss of generality we will assume that $F$ is smooth (it can be actually showed that by applying our 
techniques in the non-differentiable setting, one conducts blackbox optimization using different smooth proxies of $F$ depending on the probabilistic distributions used to 
sample perturbations).

\begin{comment}
Throughout this paper, the terms: Evolution Strategy (ES), Monte-Carlo (MC) gradient estimation, or randomized finite differences may be used interchangeably. We first present these standard methods for gradient estimation and then propose our approaches. 

\subsection{Baselines: Monte Carlo Estimators of Gradients of Smoothings}

In order to optimize blackbox function $F:\mathbb{R}^{d} \rightarrow \mathbb{R}$, one can consider computing the approximate gradient of certain smoothings of $F$. The \textit{Gaussian smoothing} \cite{nesterov} of $F$ is given as:
\begin{align}
\begin{split}
F_{\sigma}(\theta) = \mathbb{E}_{\mathbf{g} \in \mathcal{N}(0,\mathbf{I}_{d})}[F(\theta + \sigma \mathbf{g})] = \\
(2\pi)^{-\frac{d}{2}}
\int_{\mathbb{R}^{d}}F(\theta + \sigma \mathbf{g})e^{-\frac{\|\mathbf{g}\|^{2}}{2}}d\mathbf{g}
\end{split}
\end{align}
for a smoothing parameter $\sigma > 0$.
The gradient of the Gaussian smoothing of $F$ is given by the formula:
\begin{equation}
\nabla F_{\sigma}(\theta)=\frac{1}{\sigma}\mathbb{E}_{\mathbf{g} \sim \mathcal{N}(0,\mathbf{I}_{d})}[F(\theta + \sigma \mathbf{g})\mathbf{g}].    
\end{equation}

That formula leads to the straightforward unbiased Monte Carlo (MC) estimator of $\nabla F_{\sigma}(\theta)$, called \textit{vanilla ES gradient estimator} \cite{stockholm}  given by:
\begin{equation}
\widehat{\nabla}^{\mathrm{V}}_{\mathrm{MC}}F_{\sigma}(\theta) = 
\frac{1}{k\sigma}\sum_{i=1}^{k}F(\theta + \sigma \mathbf{g}_{i})\mathbf{g}_{i},
\end{equation}

where each $\mathbf{g}_{i}$ is sampled independently from $\mathcal{N}(0,\mathbf{I}_{d})$.
We call vectors $\mathbf{g}_{i}$ the perturbation (or sampling) directions.
This is the baseline estimator that random search ES methods for policy optimization rely on, in particular methods proposed in \cite{ES} and \cite{horia}. 

Different variants of that baseline method, where other control variate terms (leading to estimators that are still unbiased) as well as sensing directions $\mathbf{g}_{i}$ taken from other distributions (such as rows of random Hadamard matrices for which the corresponding estimators become biased) were proposed \cite{stockholm} \cite{montreal}. 
Here some of the most prominent examples include: the so-called \textit{forward finite-difference ES gradient estimator} given by:

\begin{equation}
\widehat{\nabla}^{\mathrm{FD}}_{\mathrm{MC}}F_{\sigma}(\theta) = 
\frac{1}{k\sigma}\sum_{i=1}^{k}(F(\theta + \sigma \mathbf{g}_{i})-F(\theta))\mathbf{g}_{i},
\end{equation}

and an \textit{antithetic ES gradient estimator} defined as:

\begin{equation}
\widehat{\nabla}^{\mathrm{AT}}_{\mathrm{MC}}F_{\sigma}(\theta) = 
\frac{1}{2k\sigma}\sum_{i=1}^{k}(F(\theta + \sigma \mathbf{g}_{i})-F(\theta - \sigma \mathbf{g}_{i}))\mathbf{g}_{i},
\end{equation}


Both different control variates (e.g. antithetic sampling) as well as different distributions for $\mathbf{g}_{i}$ (e.g. those giving rise to quasi Monte Carlo estimators of $\nabla F_{\sigma}(\theta)$) lead to moderate accuracy gains (lower variance of the estimator), but even these methods require substantial number of sensing directions (i.e. substantial number of expensive rollouts) to be capable to learn good quality RL policies.
\end{comment}

% \subsection{Robust Blackbox Optimization Algorithm}

% Assume that $F$ is smooth.
Let $\mathbf{w} \in \mathbb{R}^{d}$ and $\|\mathbf{w}\|_{2}=1$. Notice that the following holds:
\begin{equation}
\lim_{\sigma \rightarrow 0} \frac{F(\theta + \sigma \mathbf{w})-F(\theta)}{\sigma} = \nabla F(\theta)^{\top}\mathbf{w}    
\end{equation}

Thus for $\mathbf{z}$ with $\|\mathbf{z}\| \ll 1$ the following is true:
\begin{equation}
F(\theta + \mathbf{z})-F(\theta)
\approx \nabla F(\theta)^{\top} \mathbf{z}
\end{equation}

We call $F(\theta + \mathbf{z})-F(\theta)$ the \textit{forward finite-difference estimation of the action of gradient on $\mathbf{z}$}.
By the similar analysis as above, we can obtain the \textit{antithetic finite-difference estimation of the action of gradient on $\mathbf{z}$}:

\begin{equation}
\frac{F(\theta + \mathbf{z})-F(\theta - \mathbf{z})}{2}
\approx \nabla F(\theta)^{\top} \mathbf{z}
\end{equation}

With this characterization, we can formulate the problem of finding an approximate gradient $\nabla F(\theta)$ as a regression problem 
(we will choose finite-difference estimation of the action of the gradient, but completely analogous analysis can be done for the antithetic one). 

Given scalars $\{F(\theta+\mathbf{z}_{i})\}_{i=1}^{k}$ (corresponding to rewards obtained by different perturbed versions of the policy encoded by $\theta$), we formulate the 
regression problem by considering vectors $\{\mathbf{z}_{1},...,\mathbf{z}_{k}\}$ with regression values $F(\theta+\mathbf{z}_{i}) - F(\theta)$ for $i=1,...,k$. 
We propose to solve this regression task by solving the following minimization problem:
\begin{equation}
\widehat{\nabla}_{\mathrm{RBO}}F(\theta) =  
\arg \min_{\mathbf{v} \in \mathbb{R}^{d}} \frac{1}{2k}\|\mathbf{y} - \mathbf{Z}\mathbf{v}\|^{p}_{p} + \alpha \|\mathbf{v}\|^{q}_{q},    
\end{equation}
where $p, q \geq 1$, $\mathbf{Z} \in \mathbb{R}^{k \times d}$ is the matrix with rows encoding perturbations $\mathbf{z}_{i}$ and where the sequences of these rows are 
sampled from some given joint multivariate distribution $\mathbb{P} \in \mathcal{P}(\mathbb{R}^{d} \times ... \mathbb{R}^{d})$, vector $\mathbf{y} \in \mathbb{R}^{k}$ consists of regression values 
(i.e. $y_{i} = F(\theta+\mathbf{z}_{i}) - F(\theta)$ for $i=1,...,k$) and $\alpha > 0$ is a regularization parameter.

\begin{comment}
\begin{algorithm}
\textbf{Input:} $F : \Theta \rightarrow \mathbb{R}$, scaling parameter sequence $\{\delta_t \}_t$, initial $\theta_0 = \mathbf{u}_0 \in \Theta$, number of perturbations $k$, step size sequence $\{ \eta_t \}_t$, sampling distribution $\mathbb{P} \in \mathcal{P}(\mathbb{R}^{d})$, parameters $p,q,\alpha$, number of iterations $T$.  .\; \\
\textbf{Output:} Vector of parameters $\theta_{T}$.  .\; \\
\For{$t=0, 1, \ldots, T-1$}{
  1. Sample $\mathbf{g}^{(t)}_1, \cdots, \mathbf{g}^{(t)}_k$ from $\mathbb{P}$. \;\\
  2. Compute $F(\theta_t)$ and $F(\theta_t + \delta_t \mathbf{g}^{(t)}_j)$ for all $j$. \; \\
  3. Let $\mathbf{Z}_t \in \mathbb{R}^{k \times d}$ be a matrix having rows equal to the vectors $\delta_t \times \mathbf{g}^{(t)}_j$.\; \\
  4. Let $\mathbf{y}_t \in \mathbb{R}^k$ be a vector having entries equal to $F(\theta_t + \delta_t \mathbf{g}^{(t)}_j) - F(\theta_t)$.\; \\
  5. Let $\widehat{\nabla}_{\mathrm{RBO}}F(\theta)$ be the resulting vector after solving the following optimization problem:
  \begin{align*}
    \widehat{\nabla}_{\mathrm{RBO}}F(\theta) =  
    \arg \min_{\mathbf{v} \in \mathbb{R}^{d}} \frac{1}{2k}\|\mathbf{y}_{t} - \mathbf{Z}_{t}\mathbf{v}\|^{p}_{p} + \alpha \|\mathbf{v}\|^{q}_{q}, 
  \end{align*}\;\\
  6. Take $\mathbf{u}_{t+1} = \mathbf{u}_t + \eta_t \widehat{\nabla}_{\mathrm{RBO}}F(\theta)$ \; \\
  7. Take $\theta_{t+1} = \arg\max_{\theta \in \Theta} \langle \theta, \mathbf{u}_{t+1} \rangle - \frac{1}{2}\| \theta \|_2^2$. .\; \\
 }
 \caption{$\mathrm{RBO}$ Algorithm.}
\label{Alg:robust_gradient_recovery}
\end{algorithm}
\end{comment}

% \begin{comment}
\begin{algorithm}[H]
\textbf{Input:} $F : \Theta \rightarrow \mathbb{R}$, scaling parameter sequence $\{\delta_t \}_t$, initial $\theta_0 = \mathbf{u}_0 \in \Theta$, number of perturbations $k$, step size sequence $\{ \eta_t \}_t$, sampling distribution $\mathbb{P} \in \mathcal{P}(\mathbb{R}^{d})$, parameters $p,q,\alpha, \tau$, number of epochs $T$.  \; \\
\textbf{Output:} Vector of parameters $\theta_{T}$. \; \\
1. Initialize $\Theta^{\mathrm{pert}}_{\mathrm{old}} = \emptyset$, $R_{\mathrm{old}} = \emptyset$ ($|\Theta^{\mathrm{pert}}_{\mathrm{old}}|=|R_{\mathrm{old}}|$). \; \\
\For{$t=0, 1, \ldots, T-1$}{
  1. Compute all distances from $\mathbf{u}_{t}$ to $\theta^{\mathrm{pert}}_{\mathrm{old}} \in \Theta^{\mathrm{pert}}_{\mathrm{old}}$. \; \\
  2. Find the closest $\tau$-percentage of vectors from $\Theta^{\mathrm{pert}}_{\mathrm{old}}$ and call it $\Theta^{\mathrm{near}}_{\tau}$. Call the corresponding subset of $R_{\mathrm{old}}$ as $R^{\mathrm{near}}_{\tau}$. \; \\
  3. Sample $\mathbf{g}^{(t)}_1, \cdots, \mathbf{g}^{(t)}_{k-|\Theta^{\mathrm{near}}_{\tau}|}$ from $\mathbb{P}$. \;\\
  4. Compute $F(\theta_t)$ and $F(\theta_t + \delta_t \mathbf{g}^{(t)}_j)$ for all $j$. \; \\
  5. Let $\mathbf{Z}_t \in \mathbb{R}^{k \times d}$ be a matrix 
  obtained by concatenating rows given by $\delta_t \times \mathbf{g}^{(t)}_i$ and those 
  of the form: $\mathbf{p}_{i}-\theta_{t}$, where $\mathbf{p}_{i} \in \Theta^{\mathrm{near}}_{\tau}$.\; \\
  6. Let $\mathbf{y}_t \in \mathbb{R}^k$ be the vector obtained by concatenating values $F(\theta_t + \delta_t \mathbf{g}^{(t)}_j) - F(\theta_t)$ with those
  of the form: $r_{i} - F(\theta_{t})$, where $r_{i} \in R^{\mathrm{near}}_{\tau}$. \; \\
  7. Let $\widehat{\nabla}_{\mathrm{RBO}}F(\theta_t)$ be the resulting vector after solving the following optimization problem:
  \begin{align*}
    \widehat{\nabla}_{\mathrm{RBO}}F(\theta_t) =  
    \arg \min_{\mathbf{v} \in \mathbb{R}^{d}} \frac{1}{2k}\|\mathbf{y}_{t} - \mathbf{Z}_{t}\mathbf{v}\|^{p}_{p} + \alpha \|\mathbf{v}\|^{q}_{q}, 
  \end{align*}\;\\
  8. Take $\mathbf{u}_{t+1} = \theta_t + \eta_t \widehat{\nabla}_{\mathrm{RBO}}F(\theta_t)$ \; \\
  9. Take $\theta_{t+1} = \arg\max_{\theta \in \Theta} \langle \theta, \mathbf{u}_{t+1} \rangle - \frac{1}{2}\| \theta \|_2^2$.\;\\  
  10. Update $\Theta^{\mathrm{pert}}_{\mathrm{old}}$ to be the set
  of the form $\theta_{t} + \mathbf{z}_{i}$, where $\mathbf{z}_{i}$s are rows of $\mathbf{Z}_{t}$
  and $\theta_{t}$, and $R_{\mathrm{old}}$ to be the set of the corresponding values $F(\theta_{t}+\mathbf{z}_{i})$ and $F(\theta_{t})$.
 }
 \caption{Robust Blackbox Optimization Algorithm}
\label{Alg:tr-robust_gradient_recovery}
\end{algorithm}
% \end{comment}

Note that various known regression methods arise by instantiating the above optimization problems with different values of $p, q$ and $\alpha$.
In particular, $p=q=2$ leads to the ridge regression algorithm (\cite{regression}), $p=2$, $q=1$ to the Lasso method (\cite{lasso}) and $p=1$, $\alpha=0$ to LP decoding (\cite{dwork2007price}).
The latter one is especially important since it is applied in several applications ranging from dimensionality reduction techniques (\cite{tao}) to database retrieval algorithms
(\cite{dwork2007price}) and compressive sensing methods in medical imaging (\cite{ning}). 
We show empirically and theoretically that in the ES context it leads to the most robust policy learning algorithms,
insensitive to substantial adversarial noise.
Note also that as opposed to standard random search ES methods described before, perturbations $\mathbf{z}_{i}$ do not need to be taken from the Gaussian multivariate distribution and 
they do not even need to be independent. This observation will play a crucial role when we propose to reduce sampling complexity by reusing policy rollouts.

\subsection{Sliding Trust Region for ES optimization}

The main advantage of the above regression based optimization algorithms for RL blackbox function gradient approximation is that it is not necessary to sample from a fixed 
distribution at each step in order to apply them. Instead, we use the idea that at any vector $\theta$ encoding the current policy, a good quality estimator of the 
corresponding gradient can be deduced from the blackbox function at any parameter point cloud around it. 
This prompts the idea of using a trust region approach \cite{scheinberg}, where perturbations are reused from epoch to epoch. Reusing samples allows us to 
reduce sampling complexity since it reduces the number of times blackbox function $F$ is being called, e.g. the number of times the simulator is used.
We propose two simple trust region techniques for sample reuse and show that they work very well in practice (see: Section \ref{sec:exp}).
Denote by $\theta_{t+1}$ current parameter vector obtained throughout the optimization process. In the first strategy, called \textit{static trust region method}, 
all perturbed policies of the form $\theta_{t} + \delta_{t} \mathbf{g}_{j}^{t}$ for $j=1,...,k$ that are within radius $R$ from $\theta_{t+1}$ are resued to 
approximate gradient of $F$ in $\theta_{t+1}$ (where $R$ is a tuned hyperparameter). In the second strategy that we denote as \textit{dynamic trust region method}, 
only a fixed fraction $\tau$ (where $\tau$ is another hyperparameter) of policies of the form $\theta_{t} + \delta_{t} \mathbf{g}_{i}^{t}$ that are closest to $\theta_{t+1}$ are reused.


Our $\mathrm{RBO}$ algorithm taking advantage of the above techniques is presented in the $\mathrm{Algorithm}$ 1 box (we present dynamic trust region version).
At each epoch of the procedure the regularized regression problem is solved to estimate the gradient. The estimate is then used to update policy parameters.
Step $9$ in the $\mathrm{for}$-loop of the $\mathrm{RBO}$ algorithm is conducted to make sure that the resulting parameter vector is in the domain of allowed parameter vectors $\Theta$.

% Obtained in such a way, trust region method based modification of the $\mathrm{RBO}$ algorithm, called $\mathrm{TR}$-$\mathrm{RBO}$ algorithm is presented in 
% the $\mathrm{Algorithm}$ 2 box.

\begin{comment}
\subsection{$\mathrm{RBO}$ Algorithm versus Monte Carlo Methods}

The class of $\mathrm{RBO}$ algorithms contains as very special cases some of the most efficient Monte Carlo methods for blackbox function gradient estimation proposed recently in \cite{stockholm} and based on random orthogonal sensing directions $\mathbf{g}_{i}^{\mathrm{ort}}$.
There are many different ways of constructing orthogonal samples. Consider for instance a Gaussian matrix $\mathbf{G} \in \mathbb{R}^{k \times d}$ with entries taken independently at random from $\mathcal{N}(0,1)$ (we will assume here that $k \leq d$).
Perturbations $\mathbf{g}_{i}^{\mathrm{ort}}$ can be constructed by conducting Gram-Schmidt orthogonalization of $\mathbf{G}$ in order to get an orthonormal matrix $\mathbf{G}_{\mathrm{ort}}$ and then independently renormalizing rows so that the distribution of their lengths matches the distribution of the lengths of $d$-dimensional Gaussian vectors or so that the length of each row is equal to $\sqrt{d}$. 
Another construction is based on the products of the so-called \textit{random Hadamard matrices} $\mathbf{HD}$, where $\mathbf{H}$ is a Kronecker-product Hadamard matrix and $\mathbf{D}$ is a random diagonal matrix with entries taken independently at random from $\{-1,+1\}$. 
The following is true (a completely analogous statement can be obtained for the antithetic case):

\begin{lemma}
The class of ES algorithms applying Monte Carlo based forward finite-difference estimators with $k=d$ orthogonal sensing directions $\mathbf{g}_{i}^{\mathrm{ort}}$ of fixed deterministic length equal to $\sqrt{d}$ is equivalent to particular sub-classes of $\mathrm{RBO}$ algorithms with $p=q=2$ as well as with $p=1$ and $\alpha = 0$
(using forward finite-difference estimation of the action of the gradient and the same samples).
\end{lemma}

\begin{proof}
Consider first the case $p=q=2$ (ridge regression for gradient approximation). The solution to the ridge regression problem:
\begin{equation}       
\arg \min_{\mathbf{v} \in \mathbb{R}^{d}} \frac{1}{2d}\|\mathbf{y}_{t} - \mathbf{Z}_{t}\mathbf{v}\|^{2}_{2} + \alpha \|\mathbf{v}\|^{2}_{2}
\end{equation}
is of the form
\begin{equation}
\widehat{\nabla}_{\mathrm{RBO}}F_{\mathrm{ridge}}(\theta) = 
(\mathbf{Z}_{t}^{\top}\mathbf{Z}_{t} + 2d \alpha \mathbf{I}_{d})^{-1}\mathbf{Z}_{t}^{\top}\mathbf{y}_{t}
\end{equation}

Notice that from the assumptions of the lemma we get: $\mathbf{Z}_{t}\mathbf{Z}_{t}^{\top} = \delta^{2}d \mathbf{I}_{d}$. Therefore we have: $\mathbf{Z}_{t}^{\top} = \delta^{2}d\mathbf{Z}_{t}^{-1}$, thus we obtain:
\begin{equation}
\widehat{\nabla}_{\mathrm{RBO}}F_{\mathrm{ridge}}(\theta) = 
\frac{1}{d \delta} \mathbf{G}_{\mathrm{ort}}^{\top}\mathbf{y}_{t}
\cdot \frac{\delta^{2}}{\delta^{2}+2\alpha},
\end{equation}
where $\mathbf{G}_{\mathrm{ort}}^{\top}$ is a matrix with rows given by $\mathbf{g}_{i}^{\mathrm{ort}}$.
Thus if we take $\delta = \sigma_{\mathrm{MC}}$, where
$\sigma_{\mathrm{MC}}$ stands for the smoothing parameter in the MS estimator and furthermore, $\eta = \eta_{\mathrm{MC}}\frac{\delta^{2}+2\alpha}{\delta^{2}}$, where $\eta_{\mathrm{MC}}$ stands for the steps size in the algorithm using that MC estimator, then $\mathrm{RBO}$ Algorithm is equivalent to that one and the proof is completed.
Now consider the case: $p=1, \alpha = 0$.
But then (since $k=d$) 
$\widehat{\nabla}_{\mathrm{RBO}}F_{\mathrm{ridge}}(\theta)$ is a solution to the linear system and is of the form:
\begin{equation}
\widehat{\nabla}_{\mathrm{RBO}}F_{\mathrm{ridge}}(\theta) = \mathbf{Z}_{t}^{-1}\mathbf{v}=\frac{1}{d\delta} 
\mathbf{G}_{\mathrm{ort}}^{\top}\mathbf{y}_{t} \cdot \frac{1}{\delta}
\end{equation}
and we proceed as before, but this time with 
$\eta = \eta_{\mathrm{MC}}\delta$.
\end{proof}

The class of the $\mathrm{RBO}$ algorithms contains as special cases recent MC methods for blackbox optimization based on the orthogonal sensing, 
but in the next sections we will show that they outperform them. Our ($\mathrm{TR}$)-$\mathrm{RBO}$ algorithms using $p=q=2$, $p=2, q=1$ or $p=1, \alpha=0$ will 
be capable of learning good quality policies for $k \ll d$ (see: Section \ref{sec:exp}). Furthermore (as we will prove theoretically in the next section and 
confirm experimentally in Section \ref{sec:exp}), in the noisy regime setting, where lots of measurements are corrupted aribtrarily, $\mathrm{RBO}$ algorithms 
still work well as opposed to MC-based methods.
\end{comment}



==> minitaur_path_tracking.tex <==
\paragraph{\textbf{Path tracking problem for quadruped robots}}

The second task is to learn walking while staying within some specific 2D curved path (shown in black in Fig. \ref{fig:path}), 
where the path forces the robot to steer left and right. The task is much harder because the legs of the robot do not have the third degree of 
freedom which would provide the sideways motion to the legs to turn easily. 
The robot is rewarded for staying within the path boundary and moving forward. The observations include robot IMU data, 
its position and orientation. Robot's joint motor positions are output as action.
We use the same PMTG architecture as before.


\begin{figure}[!t]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{RBO}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/path_rbo_1.png}}
	\subfigure[$\mathrm{RBO}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/path_rbo_2.png}}
	\subfigure[$\mathrm{RBO}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/path_rbo_3.png}}	
	\subfigure[$\mathrm{RBO}$: phase IV]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/path_rbo_4.png}}
	\subfigure[$\mathrm{RBO}$: phase V]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/path_rbo_5.png}}
	\subfigure[$\mathrm{RBO}$: phase VI]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/path_rbo_6.png}}	
\end{minipage}
	\caption{Policy steering the quadruped to follow the path trained by the $\mathrm{RBO}$ algorithm in action. The algorithm is using only $k=170$ perturbations per epoch to train a $340$-dimensional
	policy.}
	\label{fig:path} 
\end{figure}

As for learning stable walking behaviors, $\mathrm{RBO}$ was responsible here for training a linear $340$-dimensional component of a larger hybrid policy.
We obtained similar results as before. The $\mathrm{RBO}$-policy successfully steering the robot to follow the path is presented on Fig. \ref{fig:path}.
Training curves obtained for two random seeds for this task with $\mathrm{RBO}$ are presented in Fig. \ref{fig:path-curves}. Rewards $R>7.5$ translate to good steering policies.

\begin{figure}[!t]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{RBO}$: seed I]{\includegraphics[keepaspectratio, width=0.25\textwidth]{plots-paper/final/path_curve_1.png}}
	\subfigure[$\mathrm{RBO}$: seed II]{\includegraphics[keepaspectratio, width=0.233\textwidth]{plots-paper/final/path_curve_2.png}}	
\end{minipage}
	\caption{Training curves for learning steering quadruped policies guiding the robot to follow the path. In both runs $1500$ epochs with $k=170$ perturbations
	each suffice to train policies successfully completing the task.}
	\label{fig:path-curves} 
\end{figure}


==> minitaur_walking.tex <==
\subsection{Locomotion for quadruped robots}
\label{locomotion}

We tested our algorithm on two different quadruped locomotion tasks derived from a real quadruped robot (`Minitaur' from Ghost Robotics, see: Fig. \ref{fig:real}),
with different reward functions encouraging different behaviors.
Minitaur has $4$ legs and $8$ degrees of freedom, where each leg has the ability to swing and extend to a certain degree using the PD controller 
provided with the robot. We train our policies in simulation using the pybullet environment modeled after the robot (\cite{coumans}).
To learn walking for quadrupeds, we use architectures called \textit{Policies Modulating Trajectory Generators} (PMTGs) that have been recently proposed 
in \cite{atil}. The architecture incorporates basic cyclic characteristics of the locomotion and leg movement primitives by using trajectory 
generators, a parameterized function that provides cyclic leg positions. The policy is responsible for modulating and adjusting leg trajectories as 
needed for the environment. 
% More detailed explanation about the architecture can be found in [ref pmtg].

\paragraph{\textbf{Straight walking with changing speeds}}

The robot is rewarded for walking at the desired speed which is changed during the episode. 
This task is identical to the original one tested with PMTG. More details about the environment 
such as speed profile during the episode, reward calculation as well as observation and action space definitions can be found in \cite{atil}.

\begin{figure}[!t]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{RBO}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/walking_lp4000_noise_1.png}}
	\subfigure[$\mathrm{RBO}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/walking_lp4000_noise_2.png}}
	\subfigure[$\mathrm{RBO}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/walking_lp4000_noise_3.png}}	
\end{minipage}
	\caption{A policy trained by the $\mathrm{RBO}$ algorithm in action. We used LP decoding to handle $400$ arbitrarily corrupted measurements per epoch 
	and $4000$ perturbations per epoch (giving noise level $10\%$). The training was run on a cluster of $4000$ machines, each handling one perturbation. 
	The algorithm manages to recover the gradient of the blackbox function $F$, as our theoretical results predict, and produces stable walking behaviors 
	(demonstration in the attached video). We obtained similar results for as few as only $32$ perturbations per epoch and a $25\%$ noise level which shows that
	$\mathrm{RBO}$ handles substantial noise even if $k \ll d$.}
	\label{fig:walking} 
\end{figure}

The $\mathrm{RBO}$ algorithm was compared with other methods on the task of training a linear component ($84$-dimensional policy) of the PMTG architecture.
We compared with different variants of the $\mathrm{ARS}$ algorithm (with the filtering heuristic turned on or off), since it was a method of choice in \cite{atil}.
In the noiseless setting all methods produce similar training curves
as we see in Fig. \ref{fig:walking-curves} (a). The results are very different if $25\%$ of all measurements are arbitrarily corrupted 
(Fig. \ref{fig:walking-curves} (b)). Then, $\mathrm{RBO}$ manages to learn good walking behavior much faster than $\mathrm{ARS}$. 
In that setting $\mathrm{ARS}$ with filtering turned on (used in \cite{atil}), much more sensitive to noise, does not work at all and thus we did not present it on a plot.
Results from Fig. \ref{fig:walking-curves} were obtained for $k=32$ perturbations per epoch, we had similar results for other configurations of training
(see: Fig. \ref{fig:walking}).

\begin{figure}[!t]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{Minitaur}$-noiseless]{\includegraphics[keepaspectratio, width=0.5\textwidth]{plots-paper/final/minitaur_nonoise.png}}
	\subfigure[$\mathrm{Minitaur}$-25\% noise]{\includegraphics[keepaspectratio, width=0.47\textwidth]{plots-paper/final/minitaur_noise.png}}	
\end{minipage}
	\caption{Comparison of $\mathrm{RBO}$ with other policy learning methods for learning quadruped stable walking. Even though in the noiseless
	setting all methods produce similar training curves, when noise is injected $\mathrm{RBO}$ learns stable walking policies much faster.} 
	\label{fig:walking-curves} 	
\end{figure}

==> mujoco.tex <==
\subsection{$\mathrm{OpenAI}$ $\mathrm{Gym}$ $\mathrm{mujoco}$ tasks}

We focused on the $\mathrm{mujoco}$ locomotion tasks ($\mathrm{Swimmer}$, $\mathrm{Hopper}$, $\mathrm{Walker2d}$, $\mathrm{Humanoid}$) since $\mathrm{RBO}$ 
worked particularly well on locomotion tasks for quadruped robots described in detail above. However we showed that it is not only limited to locomotion, applying it
successfully to the $\mathrm{Pusher}$ environment, where $\mathrm{ARS}$ with the similar number of perturbations per epoch did not manage to learn good quality policies.
All the plots were created by averaging over $s=5$ random seeds.

\begin{figure}[H]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{Swimmer}$-noiseless]{\includegraphics[keepaspectratio, width=0.25\textwidth]{plots-paper/final/swimmernonoise.png}}
	\subfigure[$\mathrm{Pusher}$-noiseless]{\includegraphics[keepaspectratio, width=0.24\textwidth]{plots-paper/final/pushernonoise.png}}	
\end{minipage}
	\caption{Comparison of $\mathrm{RBO}$ algorithms with other policy learning methods on $\mathrm{Swimmer}$ and 
	 $\mathrm{Pusher}$ tasks with no extra noise injected.}
	\label{fig:swimmerpusher-no-noise} 
\end{figure}

\begin{figure}[H]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{ARS}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/sw_ars_1.png}}
	\subfigure[$\mathrm{ARS}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/sw_ars_2.png}}
	\subfigure[$\mathrm{ARS}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/sw_ars_3.png}}	
	\subfigure[$\mathrm{RBO}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/sw_rbo_1.png}}
	\subfigure[$\mathrm{RBO}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/sw_rbo_2.png}}
	\subfigure[$\mathrm{RBO}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/sw_rbo_3.png}}	
\end{minipage}
	\caption{Comparison of $\mathrm{RBO}$ and $\mathrm{ARS}$ policies trained with only $k=100$ perturbations per epoch. The $\mathrm{ARS}$ policy is suboptimal
	and drives the agent to move to the side. The $\mathrm{RBO}$ policy steers the agent to efficiently move forward.}
	\label{fig:swimmer-arsrbo} 
\end{figure}

\begin{figure}[H]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{ARS}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/pu_ars_1.png}}
	\subfigure[$\mathrm{ARS}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/pu_ars_2.png}}
	\subfigure[$\mathrm{ARS}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/pu_ars_3.png}}	
	\subfigure[$\mathrm{RBO}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/pu_rbo_1.png}}
	\subfigure[$\mathrm{RBO}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/pu_rbo_2.png}}
	\subfigure[$\mathrm{RBO}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/pu_rbo_3.png}}	
\end{minipage}
	\caption{As in Fig. \ref{fig:swimmer-arsrbo}, but this time for $\mathrm{Pusher}$ environment. The $\mathrm{ARS}$ policy does not manage to
	steer the robotic arm close to the object.}
	\label{fig:pusher-arsrbo} 
\end{figure}


The first set of results is presented in Fig. \ref{fig:swimmerpusher-no-noise}, where we compare $\mathrm{RBO}$ with other methods on the $\mathrm{Swimmer}$
and $\mathrm{Pusher}$ tasks in the noiseless underconstrained setting, where the number of perturbations $k=100$ is substantially smaller than the number of parameters
of the nonlinear policy, which is $d=253$ and $d=273$ respectively. In both cases $\mathrm{RBO}$ learns effective policies whereas other methods do not.
In particular, $\mathrm{ARS}$ learns the suboptimal policy for $\mathrm{Swimmer}$, where the agent moves more to the side instead of moving forward, which we show
in the first row of Fig. \ref{fig:swimmer-arsrbo}. In the second row of Fig. \ref{fig:swimmer-arsrbo} we show the effective policy learned by $\mathrm{RBO}$.
An analogous pictorial representation of the policies learned for $\mathrm{Pusher}$ are presented in Fig. \ref{fig:pusher-arsrbo}. The $\mathrm{ARS}$ policy does not manage 
to steer the robotic arm close to the object, but the $\mathrm{RBO}$ policy does it successfully.

\begin{figure}[H]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{HalfCheetah}$-noiseless]{\includegraphics[keepaspectratio, width=0.25\textwidth]{plots-paper/final/halfcheetahnonoise.png}}
	\subfigure[$\mathrm{HalfCheetah}$-15\% noise]{\includegraphics[keepaspectratio, width=0.228\textwidth]{plots-paper/final/halfcheetahnoise.png}}	
\end{minipage}
	\caption{Comparison of $\mathrm{RBO}$ algorithm with other policy learning methods on the $\mathrm{HalfCheetah}$ task: (a) no noise injected, 
	(b): $15\%$ of all the measurements are arbitrarily corrupted.}
	\label{fig:halfcheetah} 
\end{figure}


On Fig. \ref{fig:halfcheetah} we present results for $\mathrm{HalfCheetah}$ in the noiseless and noisy setting, where as many as $15\%$ of all the measurements are 
arbitrarily corrupted. In the noiseless setting $\mathrm{RBO}$ and $\mathrm{ARS}$ provide similar training curves, being superior to $\mathrm{PPO}$ and $\mathrm{TRPO}$, 
but in the noisy setting $\mathrm{RBO}$ outperforms $\mathrm{ARS}$. All trained policies are nonlinear.

\begin{figure}[H]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{Hopper}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/ho_rbo_1.png}}
	\subfigure[$\mathrm{Hopper}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/ho_rbo_2.png}}
	\subfigure[$\mathrm{Hopper}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/ho_rbo_3.png}}	
	\subfigure[$\mathrm{Walker2d}$: phase I]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/wa_rbo_1.png}}
	\subfigure[$\mathrm{Walker2d}$: phase II]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/wa_rbo_2.png}}
	\subfigure[$\mathrm{Walker2d}$: phase III]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/wa_rbo_3.png}}	
\end{minipage}
	\caption{The first row presents the $\mathrm{RBO}$ policy learned for $\mathrm{Hopper}$ and the second row for $\mathrm{Walker2d}$. Both
	policies lead to optimal behaviors and were learned with the use of only $100$ perturbations per epoch.}
	\label{fig:howa} 
\end{figure}

\begin{figure}[H]
\begin{minipage}{1.0\textwidth}
	\subfigure[$\mathrm{Humanoid}$-noiseless]{\includegraphics[keepaspectratio, width=0.18\textwidth]{plots-paper/final/humanoid.png}}
	\subfigure[$\mathrm{Walker}$-15\% noise]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/walker.png}}
	\subfigure[$\mathrm{Hopper}$-20\% noise]{\includegraphics[keepaspectratio, width=0.16\textwidth]{plots-paper/final/hopper.png}}	
\end{minipage}
	\caption{Comparison of $\mathrm{RBO}$ with other methods on the $\mathrm{Humanoid}$, $\mathrm{Walker2d}$ and $\mathrm{Hopper}$ tasks.
	$\mathrm{RBO}$ provides clear gains for $\mathrm{Humanoid}$ (underconstrained setting, LDR-policy) and $\mathrm{Hopper}$ (overconstrained setting, 
	linear policy) with the presence of substantial noise.} 
	\label{fig:tri}
\end{figure}

In Fig. \ref{fig:tri} we present the results for three more tasks: $\mathrm{Humanoid}$, $\mathrm{Walker2d}$ and $\mathrm{Hopper}$.
For the first one we tested a noiseless setting with $k=600$ perturbations per epoch (for a $636$-dimensional LDR policy).
With these number of perturbations $\mathrm{RBO}$ learns policies getting rewards close to $5000$, outperforming $\mathrm{ARS}$.
For $\mathrm{Walker2d}$ with $15\%$ of the measurements corrupted and the same policy architecture $\mathrm{RBO}$ and $\mathrm{ARS}$ 
give similar training curves. For $\mathrm{Hopper}$ we chose a linear policy architecture which was showed
to work well for most $\mathrm{OpenAI}$ $\mathrm{Gym}$ tasks in \cite{horia} for the $\mathrm{ARS}$ algorithm. The setting is overconstrained with
$500$ perturbations per epoch. We injected substantial noise leading to $100$ measurements per epoch to be arbitrarily inaccurate. In that 
setting $\mathrm{ARS}$ does not manage to learn at all (as it is the case also for $\mathrm{PPO}$ and $\mathrm{TRPO}$ algorithms not showed on the plot), whereas 
$\mathrm{RBO}$ (using LP-decoding) learns policies with rewards $R > 1200$.

$\mathrm{RBO}$-policies in action trained with only $k=100$ perturbations per epoch for $\mathrm{Hopper}$ and $\mathrm{Walker2d}$ 
tasks with LDR nonlinear architectures of sizes $d=254$ are presented in Fig. \ref{fig:howa}. Both policies lead to optimal behaviors.








==> robust_convergence.tex <==
\section{Convergence Results for Robust Gradient Recovery}
\label{sec:robust_convergence}





In this section we provide results regarding the convergence of the 
sub-class of $\mathrm{RBO}$ algorithms with $p=1$ and $\alpha=0$
(i.e. using LP decoding to reconstruct the gradient of the blackbox function $F$) in the noisy setting. 
This noisy setting is valid in a variety of practically relevant scenarios, e.g.
in when a couple of the trajectories used during training suffer from noisy state measurements, or a constant 
fraction of the trajectories are generated via a simulator  while the remaining ones are produced in the real system, 
and when the training procedure has access to a fairly robust simulator that may substantially diverge from real dynamics 
for up to twenty three percent of all the trajectories. 
To obtain rigorous theoretical guarantees, we will need certain structural assumptions 
regarding $F$. However, as we see in Section \ref{sec:exp}, those are actually not required and furthermore other sub-classes of $\mathrm{RBO}$ 
algorithms are also capable of learning good policies.
All proofs are given in the Appendix. 

We need the following definitions. 
\begin{definition}[coefficient $\rho^{*}$]
Let $X \sim \mathcal{N}(0,1)$ and denote: $Y = |X|$. Let $f$ be the $\mathrm{pdf}$ of $Y$ and $F$ be its $\mathrm{cdf}$ function. Define $g(x)=\int_{x}^{\infty} yf(y)dy$. Function $g$ is continuous and decreasing in the interval $[0, \infty]$ and furthermore $g(0) = \mathbb{E}[Y]$. Since $\lim_{x \rightarrow \infty} g(x) = 0$, there exists $x^{*}$ such that $g(x^{*}) = \frac{\mathbb{E}[Y]}{2}$. We define $\rho^{*}$ as:
\begin{equation}
\rho^{*} = 1 - F^{-1}(x*).    
\end{equation}
Its exact numerical value is 
$\rho^{*}= 0.2390318914495168...$.
% 0.239031891449516803895...
\end{definition}

\begin{definition}[$\lambda$-smoothness]
A differentiable concave function $F: \Theta \rightarrow \mathbb{R}$ is smooth with parameter $\lambda>0$ if for every pair of points $x,y \in \Theta$:
\begin{equation*}
    \| \nabla F(y) - \nabla F(x)\|_{2} \leq \lambda \| y-x \|_2
\end{equation*}
If $F$ is twice differentiable it is equivalent to $ -\lambda I \preceq \nabla^2 F(x) \preceq 0$ for all $x \in \Theta$.
\end{definition}

\begin{definition}[$L$-Lipschitz]
We say that $F:\Theta \rightarrow \mathbb{R}$ is \emph{Lipschitz} with parameter $L>0$ if for all $x,y \in \Theta$ it satisfies $|F(x) - F(y)| \leq L \| x - y \|_2$.
\end{definition}

We are ready to state our main theoretical result.

\begin{theorem}\label{theorem::convergence_robust}
Consider a blackbox function $F:\Theta \rightarrow \mathbb{R}$. Assume that $F$ is concave, Lipschitz with parameter $L$ and smooth with smoothness parameter $\lambda$. Assume furthermore that domain $\Theta\subset \mathbb{R}^d$ is convex and has $l_2$ diameter $\mathcal{B} < \infty$. 
Consider $\mathrm{Algorithm}$ \ref{Alg:tr-robust_gradient_recovery}
with $p=1, \alpha=0, \tau = 0, \delta_t \leq \frac{L}{d\lambda \sqrt{t+1}}, \eta_t = \frac{\mathcal{B}}{L\sqrt{t+1}}$ and the noisy setting in which at each step a fraction of at most $\rho^{*}$ of all measurements $F(\theta_{t}+\delta_{t}\mathbf{g}_{j}^{t})$ are arbitrarily corrupted for $j=1,2,...,k$. 
There exists a universal constant $c_{1}>0$ such that for any $\gamma \in (0,1)$ and $T \leq \gamma \exp(c_1 d )$, the following holds
with probability at least $1-\gamma$:

%With probability $T \exp(-c_1 d)$ we have that:

\begin{equation*}
    F(\theta^*) -  \left[ \frac{1}{T} \sum_{t=0}^{T-1} F(\theta_t) \right]     \leq\frac{13}{2}\mathcal{B} L \frac{1}{\sqrt{T}},
\end{equation*}

%\note{I think we can get rid of the expectation here.}
\end{theorem}
where $\theta^{*} = \arg \max_{\theta \in \Theta} F(\theta)$. 

If $F$ presents extra curvature properties such as being strongly concave, we can get a linear convergence rate. 

\begin{definition}[Strong concavity]
A function $F:\Theta \rightarrow \mathbb{R}$ is strongly concave with parameter $\mu$ if:
\begin{equation*}
    F(y) \leq F(x) + \langle \nabla F(x), y-x \rangle - \frac{\mu}{2} \| y - x\|^2_2
\end{equation*}
\end{definition}

The following theorem holds:

\begin{theorem}\label{theorem::convergence_robust_strongconvex}
Assume conditions from Theorem \ref{theorem::convergence_robust} and furthermore that $F$ is strongly concave with parameter $\mu$. 
Take $\mathrm{Algorithm}$ \ref{Alg:tr-robust_gradient_recovery}
with $p=1, \alpha = 0, \tau = 0,  \delta_t \leq \frac{L^2}{d \mathcal{B} \mu \lambda (t+1)}, \eta_t = \frac{1}{\mu(t+1)}$ acting 
in the noisy environment in which at each step a fraction of at most $\rho^{*}$ of all measurements $F(\theta_{t}+\delta_{t}\mathbf{g}_{j}^{t})$ 
are arbitrarily corrupted for $j=1,2,...,k$. There exists a universal constant $c_{1}>0$ such that for any $\gamma \in (0,1)$ and $T \leq \gamma \exp(c_1 d )$, 
with probability at least $1-\gamma$:
\begin{equation*}
F(\theta^*) - \left[ \frac{1}{T}\sum_{t=0}^{T-1}  F(\theta_t) \right] \leq \frac{6 L^2}{\mu}\frac{(1+\log(T))}{T}.
\end{equation*}

%\note{I think we can get rid of the expectation here.}
\end{theorem}


% \begin{comment}
% \begin{algorithm}[H]
% \textbf{Input: $F : \Theta \rightarrow \mathbb{R}$, scaling parameter sequence $\{\delta_t \}_t$, initial $\theta_0 = u_0 \in \Theta$, number of perturbations $K$, step size sequence $\{ \eta_t \}_t$ \note{ The equality and definition of between $\theta_0$ and $u_0$ might not be required. } }\; \\
% %\textbf{}\;
% \For{$t=1, 2, \ldots, T$}{
%   1. Sample $v^{(t)}_1, \cdots, v^{(t)}_K$ uniformly from $\{-1,1\}^d$. \note{Leave this open to other distributions.} \;\\
%   2. $\theta_t = \arg\max_{\theta \in \Theta} \langle \theta, u_t \rangle - \frac{1}{2}\| \theta \|_2^2$.\; \\
%   3. Compute $F(\theta_t)$ and $F(\theta_t + \delta_t v^{(t)}_j)$ for $j = 1, \cdots , K$. \; \\
%   4. Let $A_t \in \mathbb{R}^{K \times d}$ be the matrix having rows equal to the vectors $\delta_t \times v^{(t)}_i$.\; \\
%   5. Let $y_t \in \mathbb{R}^K$ be the vector having entries equal to $F(\theta_t + \delta_t v^{(t)}_j) - F(\theta_t)$.\; \\
%   6. Let $\tilde{g}_t$ be the resulting $g$ vector after solving the following optimization problem:
%   \begin{align*}
%       \min_{g, y} \| y - y_t\|_1 \\
%       y_t = A_t g
%   \end{align*}\;\\
%   7. $u_{t+1} = u_t - \eta \tilde{g}_t$ \; \\
%  }
%  \caption{Robust gradient recovery.}
% \label{Alg:robust_gradient_recovery}
% \end{algorithm}
% \end{comment}



